Reasoning about Data Repetitions with Counter Systems

We study linear-time temporal logics interpreted over data words with multiple attributes. We restrict the atomic formulas to equalities of attribute values in successive positions and to repetitions of attribute values in the future or past. We demonstrate correspondences between satisfiability problems for logics and reachability-like decision problems for counter systems. We show that allowing/disallowing atomic formulas expressing repetitions of values in the past corresponds to the reachability/coverability problem in Petri nets. This gives us 2EXPSPACE upper bounds for several satisfiability problems. We prove matching lower bounds by reduction from a reachability problem for a newly introduced class of counter systems. This new class is a succinct version of vector addition systems with states in which counters are accessed via pointers, a potentially useful feature in other contexts. We strengthen further the correspondences between data logics and counter systems by characterizing the complexity of fragments, extensions and variants of the logic. For instance, we precisely characterize the relationship between the number of attributes allowed in the logic and the number of counters needed in the counter system.

==> abstract.tex <==
We study linear-time temporal logics interpreted over data words with
multiple attributes. We restrict the atomic formulas to equalities of
attribute values in successive positions and to repetitions of
attribute values in the future or past.  We demonstrate
correspondences between satisfiability problems for logics and
reachability-like decision problems for counter systems. We show that
allowing/disallowing atomic formulas expressing repetitions of values
in the past corresponds to the reachability/coverability problem in
Petri nets. This gives us \twoexpspace{} upper bounds for several
satisfiability problems.  We prove matching lower bounds by
reduction from a reachability problem for a newly introduced class of
counter systems. This new class is a succinct version of vector
addition systems with states in which counters are accessed via pointers, a
potentially useful feature in other contexts.  We strengthen further
the correspondences between data logics and counter systems by
characterizing the complexity of fragments, extensions and variants of
the logic. For instance, we precisely characterize the relationship
between the number of attributes allowed in the logic and the number
of counters needed in the counter system.
\cut{
We study linear-time temporal logics interpreted over data words 
with multiple attributes in which atomic formulas are restricted to  equalities between
values of successive positions and to repetitions of values in the future or past. 
We show correspondences between logical satisfiability problems and reachability-like
decision problems for counter systems, as the standard problems for Petri nets. 
We demonstrate that allowing/disallowing atomic formulas 
expressing past repetitions of values corresponds to the reachability/coverability problem in Petri nets. 
This gives us an 2EXPSPACE upper bounds for several logical satisfiability problems. 
We prove matching lower bounds by reduction from a reachability problem for a newly introduced class of 
counter systems (a succinct version of VASS) 
for which counters are accessed via pointers, a potentially useful feature in other contexts.
We strenghen further the correspondences between data logics and counter systems by
characterizing the complexity of fragments, extensions and variants.
For instance, we prove that reasoning about pairs of repeating values leads to 
undecidability and we characterize the complexity of 
several fragments of first-order data logics.
}

\cut{
We study the satisfiability problem of temporal logics that reason
about repetitions of values in words over infinite alphabets. We
reduce the satisfiability problem to different decision problems for
Petri nets, depending on the expressivity of the logic.

We focus on a linear temporal logic $\mainlogic$ (``Logic of
Repeating Values'') interpreted over words with multiple data in which
atomic formulae can state either local (in)equalities or
(non)repetitions of values in the future (future obligations).  The
logic $\mainlogic$ extends known logics for which satisfiability is
shown decidable by reducing them to the reachability problem for Petri
nets.  We show that adding the ability to reason about past
obligations makes the satisfiability problem equivalent to the
reachability problem for Petri nets. Without past obligations, the
satisfiability problem is equivalent to the covering problem for Petri
nets. In the reduction to the covering problem, there is an
exponential blow up. We show that this is unavoidable by formalising
the power of $\mainlogic$ to reason about subsets of variables. We
show that allowing the logic to reason about repetitions of two
variables simultaneously will lead to undecidability.
\ifLONG
We also show \pspace-completeness for several $\mainlogic$ fragments
and undecidability when repetitions of values can be done by pairs.
All the decidability and complexity results can be lifted to the case
with infinite words with multiple data or to the case with a finite
amount of MSO-definable temporal operators.  Finally, we take
advantage of these results to establish complexity results for
fragments of first-order logic over data words and to fragments of
freeze LTL with a single register. 
\else
Other results for fragments, extensions or variants are presented in
the paper. 
\fi
}


==> macros.tex <==
\newcommand{\set}[1]{\{ #1 \}}
\newcommand{\sequence}[2]{\langle #1, \ldots, #2 \rangle}
\newcommand{\couple}[2]{\langle #1,#2 \rangle}
\newcommand{\pair}[2]{\langle #1,#2 \rangle}
\newcommand{\triple}[3]{\langle #1,#2,#3 \rangle}
\newcommand{\tuple}[2]{\langle #1, \ldots, #2 \rangle}
\newcommand{\quadruple}[4]{\langle #1,#2,#3,#4 \rangle}
\newcommand{\Bool}{\ensuremath{\mathbb{B}}}
\newcommand{\Nat}{\ensuremath{\mathbb{N}}}
\newcommand{\Rat}{\ensuremath{\mathbb{Q}}}
\newcommand{\Rea}{\ensuremath{\mathbb{R}}}
\newcommand{\Zed}{\ensuremath{\mathbb{Z}}}
\newcommand{\true}{\top}
\newcommand{\false}{\perp}
\newcommand{\bottom}{\perp}
% \newcommand{\powerset}[1]{\mathcal{P}({#1})}
 \newcommand{\powerset}[1]{2^{#1}}
\newcommand{\nepowerset}[1]{\mathcal{P}^{+}({#1})}
\newcommand{\npowerset}[2]{{\cal P}^{#1}(#2)}
\newcommand{\finitepowerset}[1]{{\cal P}_f(#1)}
\newcommand{\card}[1]{{\rm card}(#1)}
\newcommand{\amap}{f}
\newcommand{\amapbis}{g}
\newcommand{\aset}{X}
\newcommand{\asetbis}{Y}
\newcommand{\asetter}{Z}
\newcommand {\length}[1] {\ensuremath{|#1|}}

% domain
\newcommand{\adomain}{D}
\newcommand{\aconcrdomain}{\mathcal{D}}


% formulae
\newcommand{\avarprop}{p}
\newcommand{\avarpropbis}{q} 
\newcommand{\avarpropter}{r} 

\newcommand{\aconstraint}{\varphi}
\newcommand{\aconstraintbis}{\psi}

\newcommand{\varprop}{\Prop} % Set of atomic propositions (for a given logic)
\newcommand{\aformula}{\phi} % a formula
\newcommand{\aformulabis}{\psi} % another formula (when at least 2 are present)
\newcommand{\aformulater}{\varphi} % another formula (when at least 3 are present)

\newcommand{\formlocal}{\aformula_{\rm local}}
\newcommand{\formnext}{\aformula_{\rm next}}
\newcommand{\formrep}{\aformula_{\rm repeat}}
\newcommand{\formupdt}{\aformula_{\rm updt}}
\newcommand{\formborder}{\aformula_{\rm border}}
\newcommand{\setdec}{Y}

\newcommand{\mynext}{{\sf X}}
\newcommand{\previous}{{\sf X}^{-1}}
\newcommand{\until}{{\sf U}}
\newcommand{\sometimes}{{\sf F}}
\newcommand{\pastsometimes}{{\sf F}^{-1}}
\newcommand{\always}{{\sf G}}
\newcommand{\since}{{\sf S}}
\newcommand{\localconj}{\overset{\circ}{\land}}

\newcommand{\ltl}{{\rm LTL}}
\newcommand{\cltl}{{\rm CLTL}}
\newcommand{\cltlfrag}[2]{\cltl^{#2}_{#1}}
\newcommand{\cctlstar}{{\rm CCTL^*}}

%%%%%%
%%%%%%

%% \newcommand{\diam}{\Diamond}
\newcommand{\diam}{\mynext \sometimes}
%% \newcommand{\dcltl}{\cltl^{\diam}}
\newcommand{\dcltl}{\mainlogic}
%% \newcommand{\ddcltl}{\cltl^{\diam,\diam^{-1}}}
\newcommand{\ddcltl}{\pmainlogic}
\newcommand{\mainlogic}{\textup{LRV}}
\newcommand{\pmainlogic}{\textup{PLRV}}
\newcommand{\dcltlm}{\textup{CLTLM}^{\diam}}

\newcommand{\fcltl}{\cltl^{\downarrow}}
\newcommand{\simcltl}{\textup{LTL}^{\downarrow}}



%%%%%%
%%%%%%


% Functions with formulae as arguments
\newcommand{\subf}[1]{sub(#1)} % set of subformulae in a broad sense
\newcommand{\cl}[1]{cl(#1)} % set of subformulae in a broad sense
\newcommand{\maxcons}[1]{maxcons(#1)}
\newcommand{\themodels}[1]{{\rm Mod}(#1)} % set of models
\newcommand{\maxexpo}[1]{{\rm exp}(#1)} % maximal exponent + 1


% Models
\newcommand{\amodel}{\sigma}
\newcommand{\asymbmodel}{\rho}


% Languages

\newcommand{\ainfword}{\sigma}
\newcommand{\aletter}{a}
\newcommand{\aletterbis}{b}
\newcommand{\aalphabet}{\Sigma}
\newcommand{\lang}[1]{{\rm L}(#1)}

% Automata
\newcommand{\aautomaton}{{\mathcal A}}
\newcommand{\aautomatonbis}{{\mathcal B}}
\newcommand{\astate}{q}
\newcommand{\states}{Q}
\newcommand{\initst}{I}
\newcommand{\finst}{F}
\newcommand{\counters}{C}
\newcommand{\ainitst}{\astate_{0}}
\newcommand{\afinst}{\astate_{f}}
\newcommand{\aconfig}{\mathit{conf}}

%Transitions
\newcommand{\aupfunc}{\vect{u}}
\newcommand{\incer}{\mathit{incer}}

% Equivalences 
\newcommand{\egdef}{\stackrel{\mbox{\begin{tiny}def\end{tiny}}}{=}} % =def=
\newcommand{\eqdef}{\stackrel{\mbox{\begin{tiny}def\end{tiny}}}{\equiv}} % =def=
\newcommand{\equivdef}{\stackrel{\mbox{\begin{tiny}def\end{tiny}}}{\equivaut}} % <=def=>
\newcommand{\equivaut}{\;\Leftrightarrow\;}


\newcommand{\step}[1]{\xrightarrow{\!\!#1\!\!}}
\newcommand{\stepinc}[1]{\xrightarrow{\!\!#1\!\!}_{\rm \small  gainy}}
\newcommand{\stepdec}[1]{\xrightarrow{\!\!#1\!\!}_{\rm \small lossy}}
\newcommand{\backstep}[1]{\xleftarrow{\!\!#1\!\!}}
\newcommand{\megastep}[1]{\xrightarrow{\!\!#1\!\!}}
\newcommand{\incstep}[1]{+\!\!\xrightarrow{\!\!#1\!\!}\!\!+}
\newcommand{\decstep}[1]{-\!\!\xrightarrow{\!\!#1\!\!}\!\!-}


% Complexity classes
\newcommand {\pspace} {\textsc{pspace}}
\newcommand {\nlogspace} {\textsc{nlogspace}}
\newcommand {\logspace} {\textsc{logspace}}
\newcommand {\expspace} {\textsc{expspace}}
\newcommand {\twoexpspace} {\textsc{2expspace}}
\newcommand {\np} {\textsc{np}}
\newcommand {\exptime} {\textsc{exptime}}
\newcommand {\polytime} {\textsc{P}}



\newcommand{\sfR}{{\sf R}}


%  Families of relations indexed by terms

\newcommand{\familybibi}[2]{(\afamilyrelation{#1})_{#1 \in #2}}
\newcommand{\afamilyrelation}[1]{R_{#1}}
\newcommand{\afamilyrelationter}[2]{R_{#2}^{#1}}
\newcommand{\afamilyrelationbis}[2]{#1_{#2}}
\newcommand{\familybis}[3]{(#1_{#2})_{#2 \in #3}}
\newcommand{\afamilyrelationq}[3]{#1_{#2}(#3)}


\newcommand{\apath}{w}
\newcommand{\apathbis}{t}
\newcommand{\anode}{n}

\newcommand{\level}[1]{{\rm lev}(#1)}
\newcommand{\nextlength}[1]{\length{#1}_{\mynext}}
\newcommand{\Terms}{{\rm Terms}}


\newcommand{\symbval}{\mathit{fr}}
% \newcommand{\symbval}{\mathit{sv}}
\newcommand{\SV}{{\rm SV}}
\newcommand{\symbmodels}{\models_{{\rm symb}}}

\newcommand{\Frame}{\mathtt{Frame}}
\newcommand{\FFrame}{\mathtt{FFrame}}
\newcommand{\numvars}{k}
\newcommand{\numcords}{k}
\newcommand{\ctridx}{i}
\newcommand{\posidx}{j}
\newcommand{\frlen}{l}
\newcommand{\finind}{i}
\newcommand{\runlen}{n}


\newcommand{\Var}{{\rm VAR}}
\newcommand{\Reg}{{\rm REG}}
\newcommand{\Prop}{{\rm PROP}} 
\newcommand{\Cons}{\mathit{Cons}}
\newcommand{\Consx}{{\rm CONS}_{x}} 
\newcommand{\Consstep}{{\rm CONS}_{\rm step}}


\newcommand{\suc}{+1}

\newcommand{\pos}{\theta}

\newcommand{\aninput}{\mathit{in}}
\newcommand{\anoutput}{\mathit{out}}

\newcommand{\unknown}{\circledast} 
\newcommand{\uset}[1]{#1^\unknown}
\newcommand{\Mod}{\mathit{Mod}}

%% A test (done on 02052012 by sd)
%% \newcommand{\vect}[1]{\overline{#1}}
\newcommand{\vect}[1]{\mathbf{#1}}

\newcommand{\Aphi}{\aautomaton_\aformula}
\newcommand{\Asymb}{\aautomaton_{\rm symb}}
\newcommand{\Asat}{\aautomaton_{\rm real}}
\newcommand{\Aosc}{\aautomaton_{\rm 1sc}}
\newcommand{\Ainc}{\aautomaton_ {\rm inc}}
\newcommand{\Adec}{\aautomaton_{\rm dec}}

%dd adding macros
\newcommand{\diff}{\ensuremath{\mathit{\,diff\,}}}
\newcommand{\union} {\ensuremath{\cup}}
\newcommand{\intersection} {\ensuremath{\cap}}
\newcommand{\nnminus} {\ensuremath{\,{\mbox{\.{-}}}\,}}
\newcommand{\nnplus} {\ensuremath{\,{\mbox{\.{+}}}\,}}
\newcommand{\dummy} {\ensuremath{\sharp}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tbc}{\fbox{
\begin{minipage}{0.25\textwidth}
  To be completed\dots
\end{minipage}
}}

\newcommand{\alang}{{\rm L}}

% a counting sequence
\newcommand{\acountseq}{\beta}
\newcommand{\acountval}{\vect{v}}

\newcommand{\afrcount}[2]{u_{#1}^{#2}}


\newcommand{\fo}[2]{{\rm FO}^{#1}(#2)}
\newcommand{\emsotwo}[2]{{\rm EMSO2}^{#1}(#2)}

\newcommand{\avariable}{\mathtt{x}}
\newcommand{\avariablebis}{\mathtt{y}}
\newcommand{\avariableter}{\mathtt{z}}
\newcommand{\defeq}{\overset{\textsf{def}}{\Leftrightarrow}}
\newcommand{\vars}{\mathtt{V}}
\newcommand{\avariablest}{s}
\newcommand{\avariabledummy}{d}

\newcommand{\defstyle}[1]{\emph{#1}}
\newcommand{\macstyle}[1]{\textbf{#1}}
\newcommand{\commstyle}[1]{\textsl{\scriptsize /* #1 */}}

%Building a satisfying model
\newcommand{\aoblfunc}{\mathit{obl}}
\newcommand{\arepfunc}{\mathit{rep}}
\newcommand{\maxnumused}{m}
\newcommand{\restr}{\upharpoonright}

%Additional notation for extended logic
\newcommand{\absymbval}{\mathit{afr}}
\newcommand{\AFrame}{\mathtt{AFrame}}
\newcommand{\Abconstr}{\Gamma_{\numvars}^{\frlen}}
\newcommand{\abconstr}{\gamma_{\numvars}^{\frlen}}
\newcommand{\partition}{\mathit{pt}}
\newcommand{\lentuple}{d}
\newcommand{\relevobls}{\vars_{\aformula}}
\newcommand{\relevobl}{v}
\newcommand{\relevctrs}{\npowerset{R}{\relevobls}}
\newcommand{\aoblset}{\chi}
\newcommand{\aoblsetbis}{\xi}
\newcommand{\aoblsetter}{\zeta}
\newcommand{\carryfwdset}{\mathtt{CF}}
\newcommand{\carryfwdel}{\mathit{cf}}
\newcommand{\localeq}{\mathit{le}}


\newcommand{\tup}[1]{\langle #1 \rangle}
\newcommand{\tupz}[1]{\left\langle #1 \right\rangle}
\newcommand{\ptup}[1]{\langle #1 \rangle^{-1}}
\newcommand{\dcltltup}{\dcltl_{\textit{vec}}}
\newcommand{\oblieq}[3]{#1 \approx \tup{#3 ?}#2}
\newcommand{\oblieqz}[3]{#1 \approx \tupz{#3 ?}#2}
\newcommand{\oblineq}[3]{#1 \not\approx \tup{#3 ?}#2}
\newcommand{\poblieq}[3]{#1 \approx \ptup{#3 ?} #2}
\newcommand{\poblineq}[3]{#1 \not\approx \ptup{#3 ?} #2}

\newcommand{\oblieqlocal}{\approx}
\newcommand{\oblineqlocal}{\not\approx}
\newcommand{\noblieqlocal}{\not\approx}


\newcommand{\N}{\Nat}
\newcommand{\Cp}{\textit{next}}
\newcommand{\Cm}{\textit{prev}}
\newcommand{\Cmin}{\textit{fst?}}
\newcommand{\Cminn}{\overline{\textit{fst}}\textit{?}}
\newcommand{\Cmax}{\textit{lst?}}
\newcommand{\Cmaxn}{\overline{\textit{lst}}\textit{?}}
\newcommand{\ICAp}{\textup{ICA}^{\!+}}
\newcommand{\ICA}{\textup{ICA}}


\newcommand{\inc}[1]{{\rm inc}(#1)}
\newcommand{\dec}[1]{{\rm dec}(#1)}
\newcommand{\zero}[1]{{\rm zero}(#1)}
\newcommand{\cnext}[1]{{\rm next}(#1)}
\newcommand{\cprevious}[1]{{\rm prev}(#1)}
\newcommand{\cisfirst}[1]{{\rm first(#1)?}}
\newcommand{\cisnotfirst}[1]{\overline{{\rm first}(#1)}{\rm ?}}
\newcommand{\cislast}[1]{{\rm last(#1)?}}
\newcommand{\cisnotlast}[1]{\overline{{\rm last}(#1)}{\rm ?}}


\newcommand{\locations}{Q}
\newcommand{\alocation}{q}
\newcommand{\alocationbis}{r}
\newcommand{\transitions}{\delta} 
\newcommand{\instructions}{I}
\newcommand{\ainstruction}{{\rm instr}}
\newcommand{\achain}{\alpha}
\newcommand{\arun}{\rho}
\newcommand{\atransition}{t}

\newcommand{\interval}[2]{[#1,#2]}
\newcommand{\acounter}{\mathtt{c}}
\newcommand{\acounterbis}{\mathtt{d}}

\newcommand{\vertuple}[4]{
  \left(
  \begin{array}{c}
    #1 \\ #2 \\ #3 \\ #4
  \end{array}
  \right)
}
\newcommand{\odd}{O}
\newcommand{\even}{E}
\newcommand{\oddin}{O_{\mathit{in}}}
\newcommand{\evenen}{E_{\mathit{fi}}}
\newcommand{\avariablebp}{\avariableter_{b}^{1}}
\newcommand{\avariableep}{\avariableter_{b}^{2}}

\newcommand{\reverse}[1]{\widetilde{#1}}
\newcommand{\aword}{u}

\newcommand{\avass}{\mathcal{A}}

\newcommand{\apcpinst}{\mathit{pcp}}

\newcounter{openproblem}
 \def\theopenproblem{\arabic{openproblem}}
\newenvironment{openproblem}{\refstepcounter{openproblem}\trivlist\item[\hskip\labelsep{Open problem \theopenproblem}.]}%
                            {\samepage\hfill\mbox{\ $\bigcirc$}\endtrivlist\par}


\newcommand{\emsot}{\textup{EMSO}\ensuremath{{}^2(+1,<,\sim)}}
\newcommand{\emsotn}{\textup{EMSO}\ensuremath{{}^2(+1,\sim)}}
\newcommand{\emsotraneq}{\textup{EMSO}\ensuremath{{}^2(<,\sim)}}
\newcommand{\emsotk}{\textup{EMSO}\ensuremath{{}^2(+1, \dotsc, +k,<,\sim)}}
\newcommand{\emsotw}{\textup{EMSO}\ensuremath{{}^2(+1,<)}}
\newcommand{\femsot}{\textit{forward-}\emsot}
\newcommand{\femsotk}{\textit{forward-}\emsotk}
\newcommand{\coloneqq}{::=}


\newcommand{\ltlplain}{\ensuremath{{\sf LTL}^\downarrow}}
\newcommand{\X}{\ensuremath{{\sf X}}}
\newcommand{\F}{\ensuremath{{\sf F}}}
\newcommand{\U}{\ensuremath{{\sf U}}}
\newcommand{\R}{\ensuremath{{\sf R}}}
\newcommand{\Xd}{\ensuremath{{\sf X}^{d}}}
\newcommand{\ltlrepeat}{\textsf{LTL}(\U, \F_=, \F_{\neq}, \set{\X^k_=, \X^k_{\neq}}_{k \in \Nat})}
\newcommand{\G}{\ensuremath{{\sf G}}}

\newcommand{\cut}[1]{}

\newcommand{\D}{\mathbb{D}}

\newcommand{\pcpdir}{MPCP$^{\textit{dir}}$}
\newcommand{\minupfunc}{\mathit{minup}}
\newcommand{\SAT}[1]{{\rm SAT(}#1{\rm )}}

\newcommand{\size}[1]{| #1 |}

\newcommand{\variabs}{\textit{vars}}
\newcommand{\subft}[1]{\textit{sub}_{\tup{ }}\!(#1)}

\newcommand{\mainlogiceq}{\mainlogic^\approx}
\newcommand{\pmainlogiceq}{\pmainlogic^\approx}

\newcommand{\adataword}{\mathfrak{dw}}
\newcommand{\adatum}{\mathfrak{d}}
\newcommand{\adatumbis}{\mathfrak{e}}

\newcommand{\maxupfunc}{\mathit{maxup}}

\newcommand{\counternb}{D}

==> tikzmacros.tex <==
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{shapes.geometric}

\newlength{\ml}
\setlength{\ml}{1cm}

\tikzstyle{atom}=[rectangle split, rectangle split draw splits =
false, rectangle split ignore empty parts, draw=black, rounded
corners=0.05\ml, minimum width=0.4\ml, inner sep=0.05\ml]

\tikzstyle{state}=[rectangle, draw=black, rounded corners=0.05\ml,
minimum width=0.4\ml, minimum height=0.2\ml]

\tikzstyle{flchop}=[rectangle, draw=black, rounded corners=0.05\ml,
minimum width=0.4\ml, minimum height=0.2\ml]

\tikzstyle{flchcnd}=[diamond, draw=black, aspect=2]

\tikzstyle{traceop}=[rectangle, draw=black,
minimum width=0.4\ml, minimum height=0.2\ml]

